Evaluating Data Influence in Meta Learning

As one of the most fundamental models, meta learning aims to effectively address few-shot learning challenges. However, it still faces significant issues related to the training data, such as training inefficiencies due to numerous low-contribution tasks in large datasets and substantial noise from incorrect labels. Thus, training data attribution methods are needed for meta learning. However, the dual-layer structure of mata learning complicates the modeling of training data contributions because of the interdependent influence between meta-parameters and task-specific parameters, making existing data influence evaluation tools inapplicable or inaccurate. To address these challenges, based on the influence function, we propose a general data attribution evaluation framework for meta-learning within the bilevel optimization framework. Our approach introduces task influence functions (task-IF) and instance influence functions (instance-IF) to accurately assess the impact of specific tasks and individual data points in closed forms. This framework comprehensively models data contributions across both the inner and outer training processes, capturing the direct effects of data points on meta-parameters as well as their indirect influence through task-specific parameters. We also provide several strategies to enhance computational efficiency and scalability. Experimental results demonstrate the framework's effectiveness in training data evaluation via several downstream tasks.

==> section/app/app_EK-FAC.tex <==
\subsection{EK-FAC}
We utilize EK-FAC to perform an approximation for $H_{i, \text{in}}$, and then compute the inversion efficiently. Revising the definition of $H_{i, \text{in}}$:
$$H_{i, \text{in}} = \partial_{\theta}\partial_{\theta} L_I(\lambda^*, \theta_i(\lambda^*);\mathcal{D}^{tr}_i).$$
The EK-FAC method relies on two approximations of the Fisher information matrix $G_{{\theta}}$, which is equivalent to $H_{i,\text{in}}$ when the loss function $\ell$ in $L_I(\lambda^*, \theta_i(\lambda^*);\mathcal{D}^{tr}_i)$ is specified as cross-entropy. Firstly, assume that the derivatives of the weights in different layers are uncorrelated, which implies that $H_{i,\text{in}}$ has a block-diagonal structure.

Suppose model $\hat{f}_\theta$ can be denoted by $\hat{f}_{\theta}(x) = f_{\theta_L} \circ \cdots \circ f_{\theta_1}(x)$. We fold the bias into the weights and vectorize the parameters in the $l$-th layer into a vector $\theta_{l}\in\mathbb{R}^{d_l}$, $d_l\in \mathbb{N}$ is the number of $l$-th layer parameters.  


Then $G_{{\theta}}$ can be replaced by $\left(G_1({\theta}), \cdots, G_L({\theta})\right)$, where 
$$G_l({\theta}) \triangleq n^{-1}\sum_{i=1}^n\nabla_{{\theta}_l}L_I(\lambda^*, \theta_i(\lambda^*);\mathcal{D}^{tr}_i) \nabla_{\theta_l}L_I(\lambda^*, \theta_i(\lambda^*);\mathcal{D}^{tr}_i)^{\mathrm{T}}.$$ 
Denote $h_{l}$, $o_l$ as the output and pre-activated output of $l$-th layer. 
Define ${\Omega}_{l-1} = \hat{G}_l(\theta) \triangleq \frac{1}{n} \sum_{i=1}^{n} h_{l-1}\left(x_{i}\right) h_{l-1}\left(x_{i}\right)^{T} \otimes \frac{1}{n} \sum_{i=1}^{n} \nabla_{o_{l}} \ell_{i} \nabla_{o_{l}} \ell_{i}^{T}$.
Then $G_l(\theta)$ can be approximated by
\begin{equation*}
{G}_l(\theta) \approx {\Omega}_{l-1}\otimes {\Gamma_{l}}.
\end{equation*}
Furthermore, in order to accelerate transpose operation and introduce the damping term, perform eigenvalue decomposition of matrix ${\Omega}_{l-1}$ and ${\Gamma_{l}}$ and obtain the corresponding decomposition results as $Q_{\Omega} {\Lambda}_{{\Omega}} {Q}_{{\Omega}}^{\top}$ and ${Q}_{\Gamma}{\Lambda}_{\Gamma} {Q}_{\Gamma}^{\top}$. Then the inverse of $ \hat{H}_l(\theta)$ can be obtained by
\begin{equation}\label{app:ekfac:1}
     \hat{H}_l(\theta)^{-1} \approx \left(\hat{G}_{l}\left(\hat{g}\right)+\lambda_{l} I_{d_{l}}\right)^{-1}=\left(Q_{\Omega_{l-1}} \otimes Q_{\Gamma_{l}}\right)\left(\Lambda_{\Omega_{l-1}} \otimes \Lambda_{\Gamma_{l}}+\lambda_{l} I_{d_{l}}\right)^{-1}\left(Q_{\Omega_{l-1}} \otimes Q_{\Gamma_{l}}\right)^{\mathrm{T}}.
\end{equation}
Besides, \citet{george2018fast} proposed a new method that corrects the error in equation \ref{app:ekfac:1} which sets the $i$-th diagonal element of $\Lambda_{\Omega_{l-1}} \otimes \Lambda_{\Gamma_{l}}$ as $\Lambda_{ii}^{*} = n^{-1} \sum_{j =1}^n \left( \left( Q_{\Omega_{l-1}}\otimes Q_{\Gamma_{l}}\right)\nabla_{\theta_l}\ell_j\right)^2_i.$\\
